The Explicit Definition of Quantifiers via Hilbert's epsilon is Confluent and Terminating

We investigate the elimination of quantifiers in first-order formulas via Hilbert's epsilon-operator (or -binder), following Bernays' explicit definitions of the existential and the universal quantifier symbol by means of epsilon-terms. This elimination has its first explicit occurrence in the proof of the first epsilon-theorem in Hilbert-Bernays in 1939. We think that there is a lacuna in this proof w.r.t. this elimination, related to the erroneous assumption that explicit definitions always terminate. Surprisingly, to the best of our knowledge, nobody ever proved confluence or termination for this elimination procedure. Even myths on non-confluence and the openness of the termination problem are circulating. We show confluence and termination of this elimination procedure by means of a direct, straightforward, and easily verifiable proof, based on a new theorem on how to obtain termination from weak normalization.

==> headerhot.tex <==
\def\subsubsubsection{\paragraph}
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\font\sixsf  = cmss10 scaled 600
\font\fvesf  = cmss10 scaled 500
%\font\sevsf  = cmss10 scaled 700
\font\egtsf  = cmss10 scaled 800
%\font\twfvit  = cmti10   \@magscale5 % text italic

\def\xiipt{\textfont\z@\twlrm 
  \scriptfont\z@\egtrm \scriptscriptfont\z@\sixrm
\textfont\@ne\twlmi \scriptfont\@ne\egtmi \scriptscriptfont\@ne\sixmi
\textfont\tw@\twlsy \scriptfont\tw@\egtsy \scriptscriptfont\tw@\sixsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
          \textfont\@ne\twlmi 
          \textfont\tw@\twlsy \textfont\lyfam\twlly
          \@boldfalse}\@boldfalse
\def\boldmath{\@ifundefined{twlmib}{\global\font\twlmib\@mbi\@magscale1\global
        \font\twlsyb\@mbsy \@magscale1\global\font
         \twllyb\@lasyb\@magscale1\relax\@addfontinfo\@xiipt
              {\def\boldmath{\everymath
                {\mit}\everydisplay{\mit}\@prtct\@nomathbold
                \textfont\@ne\twlmib \textfont\tw@\twlsyb 
                \textfont\lyfam\twllyb\@prtct\@boldtrue}}}{}\@xiipt\boldmath}%
\def\prm{\fam\z@\twlrm}%
\def\pit{\fam\itfam\twlit}\textfont\itfam\twlit \scriptfont\itfam\egtit
   \scriptscriptfont\itfam\sevit
\def\psl{\fam\slfam\twlsl}\textfont\slfam\twlsl 
     \scriptfont\slfam\tensl \scriptscriptfont\slfam\tensl
\def\pbf{\fam\bffam\twlbf}\textfont\bffam\twlbf 
   \scriptfont\bffam\ninbf \scriptscriptfont\bffam\ninbf 
\def\ptt{\fam\ttfam\twltt}\textfont\ttfam\twltt
   \scriptfont\ttfam\nintt \scriptscriptfont\ttfam\nintt 
\def\psf{\fam\sffam\twlsf}\textfont\sffam\twlsf
    \scriptfont\sffam\egtsf \scriptscriptfont\sffam\sixsf
\def\psc{\@getfont\psc\scfam\@xiipt{\@mcsc\@magscale1}}%
\def\ly{\fam\lyfam\twlly}\textfont\lyfam\twlly 
   \scriptfont\lyfam\egtly \scriptscriptfont\lyfam\sixly
 \@setstrut \rm}

\def\xxvpt{\textfont\z@\twfvrm 
  \scriptfont\z@\twtyrm \scriptscriptfont\z@\svtnrm
\textfont\@ne\twtymi \scriptfont\@ne\twtymi \scriptscriptfont\@ne\svtnmi
\textfont\tw@\twtysy \scriptfont\tw@\twtysy \scriptscriptfont\tw@\svtnsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
        \textfont\@ne\twtymi \textfont\tw@\twtysy \textfont\lyfam\twtyly
        \@boldfalse}\@boldfalse
\def\boldmath{\@subfont\boldmath\unboldmath}%
\def\prm{\fam\z@\twfvrm}%
\def\pit{\fam\z@\twfvit}%
\def\psl{\@subfont\sl\rm}%
\def\pbf{\@getfont\pbf\bffam\@xxvpt{cmbx10\@magscale5}}%
\def\ptt{\@subfont\tt\rm}%
\def\psf{\@subfont\sf\rm}%
\def\psc{\@subfont\sc\rm}%
\def\ly{\fam\lyfam\twtyly}\textfont\lyfam\twtyly 
   \scriptfont\lyfam\twtyly \scriptscriptfont\lyfam\svtnly 
\@setstrut \rm}

\catcode`\@=12


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUPERCOMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following redefines the latex macro \math not because 
% \math makes trouble but rather because I dont like it
\long\def\math#1{\relax\ifmmode{#1}\else$#1 $\fi}
%                                          ^ 
% This blank is necessary because otherwise \math{} may expand to $$
% which is different from $ $ insofar as it starts a displaymath environment 
\long\def\nomath#1{\relax\ifmmode\mbox{#1}\else{#1}\fi}
\newcommand\nlbmath[1]{\nolinebreak\math{#1}}
\newcommand\maths[2]{\math{#1#2}}
\newcommand\nlbmaths[2]{\nolinebreak\math{#1#2}}
%The fol. defines \mathcommand to work like \newcommand with the exception of 
%switching to math-mode iff the command is not called in math-mode.
%\remathcommand is like \renewcommand.

\catcode`\@=11

\long\def\@reargdefmath#1[#2]#3{\@reargdef#1[#2]{\math{#3}}}

\long\def\@argdefmath#1[#2]#3{\@ifdefinable #1{\@reargdefmath#1[#2]{#3}}}

\def\mathcommand#1{\@ifnextchar [{\@argdefmath#1}{\@argdefmath#1[0]}}

\def\remathcommand#1{\edef\@tempa{\expandafter\@cdr\string
  #1\@nil}\@ifundefined{\@tempa}{\@latexerr{\string#1\space undefined}\@ehc
    }{}\@ifnextchar [{\@reargdefmath#1}{\@reargdefmath#1[0]}}

\catcode`\@=12

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mathapplycommand      
#1#2{\mathcommand{#1}[1]{{#2}({##1})}}
\def\mathdoubleapplycommand
#1#2{\mathcommand{#1}[2]{{#2}({##1},{##2})}}
\def\mathtripleapplycommand
#1#2{\mathcommand{#1}[3]{{#2}({##1},{##2},{##3})}}
%example: \mathapplycommand\foo{\rm rubbish}
%         \foo{x} 
%produces:
%         rubbish(x)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\mathoverline=\overline
\remathcommand\overline[1]{\mathoverline{#1}}
% This makes \overline more intelligent, namely switching into math-mode
% if use in text-mode

\newcommand\mycomment[1]{{\iffalse{#1}\fi}}
% The argument of \comment is completely ignored

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting basics (lengths, struts) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setlength{\parindent}{2.0em}
\newlength{\disp}
\setlength{\disp}{\textwidth}
\addtolength{\disp}{-2.0\parindent}

\newlength{\textwidthminustwomm}
\setlength{\textwidthminustwomm}{\textwidth}
\addtolength{\textwidthminustwomm}{-0.2cm}

\newlength{\textwidthminushalfcm}
\setlength{\textwidthminushalfcm}{\textwidth}
\addtolength{\textwidthminushalfcm}{-0.5cm}

\newlength{\textwidthminusonecm}
\setlength{\textwidthminusonecm}{\textwidth}
\addtolength{\textwidthminusonecm}{-1.0cm}

\newlength{\textwidthminustwocm}
\setlength{\textwidthminustwocm}{\textwidth}
\addtolength{\textwidthminustwocm}{-2.0cm}

\newlength{\textwidthminusfourcm}
\setlength{\textwidthminusfourcm}{\textwidthminustwocm}
\addtolength{\textwidthminusfourcm}{-2.0cm}

\newlength{\textwidthminussixcm}
\setlength{\textwidthminussixcm}{\textwidth}
\addtolength{\textwidthminussixcm}{-6.0cm}

\newcommand\notop   {\vspace{-1.0\topsep}}
\newcommand\yestop  {\vspace{\topsep}}
\newcommand\halftop {\vspace{0.5\topsep}}
\newcommand\eighthtop{\vspace{0.125\topsep}}
\newcommand\ohyestop{\vspace*{\topsep}}
\newcommand\noitem  {\vspace{-1.0\itemsep}}
\newcommand\yesitem {\vspace{\itemsep}}

\newcommand\schweinerei{
\topsep 4pt plus 1pt minus 2pt
\partopsep 2pt plus 1pt minus 1pt
\renewcommand{\baselinestretch}{0.96}
\hfuzz=4pt}



\newcommand\bigmath[1]{\ \math{#1}\ }
\newcommand\bigmaths[2]{\ \math{#1}#2\ }
\newcommand\mathnlb[2]{\mbox{\math{#1}#2}}
\newcommand\bigmathnlb[2]{\ \mathnlb{#1}{#2}\ }
\newcommand\nlmath{$\hfill\mbox{}\\\mbox{}\hfill$}
\newcommand\nlnomath{\hfill\mbox{}\\\mbox{}\hfill}

%Dont include spaces for pretty print here
\newcommand\linemath[1]{\mbox{}\hfill$#1$\hfill\mbox{}\\}  
\newcommand\linemaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}\\}  
\newcommand\linenomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}\\}  
%Dont include spaces for pretty print here
\newcommand\LINEmath[1]{\mbox{}\hfill$#1$\hfill\mbox{}}
\newcommand\LINEmaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}}
\newcommand\LINEnomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}}
%Dont include spaces for pretty print here

\newcommand\mysection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{section}{#1}}
\newcommand\mysubsection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{subsection}{#1}}
\newcommand\mysubsubsection
[1]{\noindent{\bf#1}\addcontentsline{toc}{subsubsection}{#1}}

\newcommand\knuthquotation[2]
{{\footnotesize\begin{flushright}{\sl#1\par}{\noindent\sc--- #2}\end
{flushright}}}

% The fol. \par\noindent\initial{A} writes an initial letter A 
% Note that it was designed to have the bottom line exactly on
% the bottom line of the line it starts. So it works well with
%   \initial{\underline{\underline{\underline{\underline{First case:}}}}}
%   In the first case we have the following...
% The two texts "first case" share their bottom. The underline extends
% below it.
% If you do not want your intials to get the bottom line
% from the bottom line of the first but of the second line
% you must design another macro or use \initial{\raisebox{-3.5ex}{...}}

\newbox\yinibox
\def\initial#1{\par
\noindent
\setbox\yinibox\hbox{#1}%
\setbox\yinibox\vbox to \ht\yinibox{\offinterlineskip\hbox{{#1}~~}\vss}%
\leavevmode
\hangindent=\wd\yinibox
\hangafter=-2
\hbox to0pt{\hskip-\hangindent\box\yinibox\hfill}\ignorespaces}
   
%%% Parentheses: %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\inparentheses[1]{\left(\begin{array}[c]{l}#1\end{array}\right)}
\mathcommand\inbracketstight
[1]{\left[\begin{array}[c]{@{}l@{}}#1\end{array}\right]}
\mathcommand\inbrackets[1]{\left[\begin{array}[c]{l}#1\end{array}\right]}
\mathcommand\inbraces[1]{\left\{\begin{array}[c]{l}#1\end{array}\right\}}
\mathcommand\inbracestight
[1]{\left\{\begin{array}[c]{@{}l@{}}#1\end{array}\right\}}
\mathcommand\inparenthesestight
[1]{\left (\begin{array}[c]{@{}l@{}}#1\end{array}\right )}
\mathcommand\inparenthesesinline[1]{(\ #1\ )}
\mathcommand\inpit[1]{(#1)}
\mathcommand\inbracesit[1]{\{#1\}}
\mathcommand\inparenthesesinlinetight[1]{\inpit{#1}}
\newcommand\mathinparenthesesinlinetight[1]{(#1)}%allows line breaking
\mathcommand\noparenthesesoplist[1]
{{\begin{array}{r l}\relax&#1\\\end{array}}}
\mathcommand\noparenthesesoplisttop[1]
{{\begin{array}[t]{r l}\relax&#1\\\end{array}}}
\mathcommand\inparenthesesoplist[1]
{{\left(\noparenthesesoplist{#1}\right)}}
\mathcommand\inbracesoplist[1]
{{\left\{\noparenthesesoplist{#1}\right\}}}
\mathcommand\inbracketsoplist[1]
{{\left[\noparenthesesoplist{#1}\right]}}
\newcommand\oplistund        {\\\tightund        &}
\newcommand\oplistoder       {\\\tightoder       &}
\newcommand\oplistcup        {\\\tightcup        &}
\newcommand\oplistuplus      {\\\tightuplus      &}
\newcommand\oplistequivalent {\\\tightequivalent &}
\newcommand\oplistimplies    {\\\tightimplies    &}
\newcommand\oplistcirc       {\\\tightcirc       &}
\newcommand\oplistantiimplies{\\\tightantiimplies&}
\newcommand\oplistnl         {\\                 &}
\mathcommand\inparenthesesimplies[2]{{\left(\begin{array}{l l}
\multicolumn{2}{l}{#1}\\\tightimplies&#2\\\end{array}\right)}}
\newcommand\inparenthesesimpliestoplevel[3]
{\math{#1\left(\begin{array}{l}\majorheadroom\footroom#2
 \\\end{array}\right.}\\\getittotheright{\math{
 \left.\begin{array}{l l}\tightimplies&\majorheadroom\footroom#3
 \\\end{array}\right)}}} 

\newcommand\opta{{\rm[}}
\newcommand\opte{{\rm]}}
\newcommand\opt[1]{\opta#1\/\opte}
\mathcommand\displayopt
[1]{\left[\begin{array}[t]{@{\,}c@{\,}}#1\end{array}\right]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATH NOTATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\stopq{\math{.}\penalty-1\relax\,\,} %\penalty-10 is too low
\mathcommand\hastype[2]{{#1}:\,{#2}}
\mathcommand\tighthastype[2]{{#1}\tight:{#2}}
\mathcommand\prettytighthastype[2]{{#1}\,\tight:\:{#2}}
\mathcommand\typed[3]{#1\hastype{#2}{#3}\stopq}
\mathcommand\comma{,\ \ }
\mathcommand\setwithstart{\{\ }
\newcommand\setwithmark{~\math|\penalty-9\relax\,\ } 
%\penalty-10 is too low, \penalty-1 is too high
\mathcommand\setwithmarkq[1] {\ |_{#1}\ }
\mathcommand\setwithstop     {\ \}}
\newcommand\setwith
[2]{\math{\setwithstart#1}\setwithmark\math{#2\setwithstop}}
%should not be mathcommand for enabling \penalty-1
\mathcommand\displaysetwith
[2]{{\left\{\begin{array}{@{\ \ }l@{\ \ }|@{\ \ }l@{\ \ }}#1&#2\\\end
{array}\right\}}}
\mathcommand\displayset
[1]{{\left\{\begin{array}{@{\ \ }l@{\ \ }}#1\\\end{array}\right\}}}

\newcommand\tight[1]{\math{#1}}
\newcommand\tightsubseteq   {\tight\subseteq  }
\newcommand\tightnotsubseteq{\tight\nsubseteq }
\newcommand\tightsuperseteq {\tight\superseteq}
\newcommand\tightsetminus   {\tight\setminus  }
\newcommand\tightplus       {\tight+          }
\newcommand\tighttimes      {\tight\times     }
\newcommand\tightcap        {\tight\cap       }
\newcommand\tightcup        {\tight\cup       }
\newcommand\tightuplus      {\tight\uplus     }
\newcommand\tightcirc       {\tight\circ      }
\newcommand\tightin         {\tight{\,\in\,}  }
\newcommand\tightnotin      {\tight{\,\not\in\,}  }
\newcommand\tightni         {\tight{\,\ni\,}  }
\newcommand\tightnotni      {\tight{\,\not\ni\,}  }
\newcommand\tightequal      {\tight{\,=\,}\penalty-1\relax}
\newcommand\tightnotequal   {\tight{\,\not=\,}}
\newcommand\tightpreceq     {\tight{\,\preceq\,}}
\newcommand\tightprec       {\tight{\,\prec\,}}
\newcommand\tightnotprec    {\tight{\,\nprec\,}}
\newcommand\tightsucceq     {\tight{\,\succeq\,}}
\newcommand\tightsucc       {\tight{\,\succ\,}}
\newcommand\tightgtr        {\tight{\,>\,}}
\newcommand\tightless       {\tight{\,<\,}}
\newcommand\tightleq        {\tight{\,\leq\,}}
\newcommand\tightgeq        {\tight{\,\geq\,}}

\newcommand\boldequal  {\tight=}
\newcommand\boldunequal{\tight{\not=}}
\newcommand\boldless   {\tight<}
\newcommand\boldnotless{\tight{\not<}}
\newcommand\boldimplies{\tight\tightimplies}
\newcommand\Defnombox{{\rm Def}}
\newcommand\Def{\mbox{\Defnombox}}
\mathcommand\DEF{\Defnombox\:}

%\mathcommand\tightimplies{\rightarrow}    
%\mathcommand\tightantiimplies{\leftarrow}
%\mathcommand\tightequivalent{\leftrightarrow}
\mathcommand\tightimplies{\Rightarrow}
\mathcommand\tightantiimplies{\Leftarrow}
\mathcommand\tightequivalent {\Leftrightarrow}
% The one-line arrow for implication is preferable for the following reasons:
% (1) Hilbert & Bernays uses this symbol.
% (2) In intuitionistic logic, (A->B) can be seen as
%     The type of functions that transform a proof of A
%     to a proof of B, and the implication is valid,
%     if such a function exists.
% The two-line arrow is preferable for the following reason:
% (A) It is more readable in formulas with type declarations and 
%     with \mapsto as a symbol for substitution. Note that the replacement
%     of "x\mapsto y" with "y/x" has two problems again:
%     (a) This would cost me a week to replace it in all contexts.
%     (b) Readability is destroyed by the replacement, because some idiots
%         use "x/y" instead of "y/x".   
% (B) The equivalence looks more like "=" which it actually is.
\mathcommand\tightund        {\wedge}
\mathcommand\tightoder       {\vee}
\mathcommand\tightshefferstroke
% {|}
%Peckhaus: Sheffer stroke sollte größer und fetter sein, etwa mit dem TeX-Befehl \mid (oder verwenden sie ihn schon?).
{\mid}
\mathcommand\tightuparrow{\uparrow}
\def       \implies      {\ \tightimplies      \penalty-2\relax\ }
\newcommand\und          {\ \tightund          \penalty-2\relax\ }
\newcommand\oder         {\ \tightoder         \penalty-2\relax\ }
\newcommand\antiimplies  {\ \tightantiimplies  \penalty-2\relax\ }
\newcommand\equivalent   {\ \tightequivalent   \penalty-2\relax\ }
\newcommand\shefferstroke{\ \tightshefferstroke\penalty-2\relax\ }

\newcommand \id          {{\rm id}}
\mathcommand\allall      {\mathcal{V}}
\mathcommand\allsets     {\POWER\allall}
\mathcommand\allfinitesets{\FINITE\allall}
\mathcommand\urelements  {\mathcal{U}}
\mathcommand\algebra     {\mathcal{A}}
\mathcommand\balgebra    {\mathcal{B}}
\mathcommand\calgebra    {\mathcal{C}}
\mathcommand\dalgebra    {\mathcal{D}}
\mathcommand\ialgebra    {\mathcal{I}}
\mathcommand\salgebra    {\mathcal{S}}
\mathcommand\walgebra    {\mathcal{W}}
\mathcommand\ralgebra    {\mathcal{R}}
\mathcommand\algebraprime{\mathcal{A}'}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathapplycommand\FLD        {\rm field}
\mathapplycommand\DOM        {\rm dom}
\mathapplycommand\RAN        {\rm ran}
\mathapplycommand\kernel     {\rm ker}
% \mathapplycommand\FINITE     {\mbox{\fraknomath P}_\N}%for \frak from german
% \mathapplycommand\POWER      {\mbox{\fraknomath P}}
% \mathapplycommand\posfinPOWER{\mbox{\fraknomath P}_\posN\!}
\mathapplycommand\FINITE     {{\mathfrak P}_{\scriptscriptstyle\N}}%for \frak from amssymb
\mathcommand\POWERSYM        {{\mathfrak P}}
\mathapplycommand\POWER      {\POWERSYM}
\mathapplycommand\posfinPOWER{\POWERSYM_{\scriptscriptstyle\posN\!}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\CARD[1]         {\,|{#1}|\,}
\mathcommand\FLOOR[1]        {\ \lfloor#1\rfloor\ }
\mathcommand\CEIL[1]         {\ \lceil#1\rceil\ }
\mathcommand\reverserelation[1]{{#1}^{-1}}
%\mathcommand\restrictedto[1]{|_{#1}}
\mathcommand\domres[2]{{_{#2}\!\tight\upharpoonleft#1}}
\mathcommand\ranres[2]{{#1\tight\upharpoonright\!_{#2}}}
\mathcommand\funarg[1]{(#1)}
\mathcommand\app[2]{#1(#2)}
\mathcommand\displayapp[2]{#1\inparentheses{#2}}
\mathcommand\displayapptight[2]{#1\inparenthesestight{#2}}
\mathcommand\apptotuple[2]{#1#2}
\mathcommand\relapp[2]{\langle#2\rangle#1}
\mathcommand\displayrelapp
[2]{\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle\!#1}
\mathcommand\relappsin[2]{\relapp{#1}{\!\{#2\}\!}}
\mathcommand\revrelapp[2]{#1\langle#2\rangle}
\mathcommand\displayrevrelapp
[2]{#1\!\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle}
\mathcommand\revrelappsin[2]{\revrelapp{#1}{\!\{#2\}\!}}
\mathcommand\displayrevrelappsin[2]{\displayrevrelapp{#1}{\!\left\{#2\right\}\!}}
\mathcommand\pair[2]{(#1,#2)}
\mathcommand\displaypair[2]{\inparentheses{#1,\ \ #2}}
\mathcommand\displaypairtight[2]{\inparenthesestight{#1,\ \ #2}}
\mathcommand\trip[3]{(#1,#2,#3)}
\mathcommand\displaytrip[3]{\inparentheses{#1,\ \ #2,\ \ #3}}
\mathcommand\superdisplaytrip[3]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\\end{array}\right)}
\mathcommand\quar[4]{(#1,#2,#3,#4)}
\mathcommand\displayquar[4]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4}}
\mathcommand\superdisplayquar[4]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\#4\\\end{array}\right)}
\mathcommand\superdisplayquartight[4]{\left(\begin
{array}{@{}l@{}}#1,\\#2,\\#3,\\#4\\\end{array}\right)}
\mathcommand\quin[5]{(#1,#2,#3,#4,#5)}
\mathcommand\displayquin[5]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4,\ \ #5}}
\mathcommand\sext[6]{(#1,#2,#3,#4,#5,#6)}
\mathcommand\sept[7]{(#1,#2,#3,#4,#5,#6,#7)}
\mathcommand\oct[8]{(#1,#2,#3,#4,#5,#6,#7,#8)}
\mathcommand\ninetuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9)}
\newcommand\tentuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\singletonrest}
\newcommand\singletonrest[1]{#1)}
\newcommand\elev[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\pairrest}
\newcommand\pairrest[2]{#1,#2)}
\mathcommand\setwithq[3]     {\setwithstart#2\setwithmarkq{#1}#3\setwithstop}
\mathcommand\setofwords[1]{#1^{\textstyle\ast}}
\mathcommand\setofwordsscriptstyle[1]{#1^{\ast}}
\mathcommand\setofnonemptywords[1]{#1^+}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\FUNSET   [2]{{#1}\rightarrow{#2}}
\mathcommand\PARFUNSET[2]{{#1}\leadsto   {#2}}
\mathcommand\FUNDEF   [3]{\hastype{#1}{\FUNSET   {#2}{#3}}}
\mathcommand\PARFUNDEF[3]{\hastype{#1}{\PARFUNSET{#2}{#3}}}
%categories
\mathcommand\morphcolon{::}
\mathcommand\morpharrow{\rightarrow}
\mathcommand\morph  [3]{{#1}\morphcolon{#2}\morpharrow{#3}}
\newcommand\Idname{{\rm Id}}
\mathcommand\Id[1]{{\Idname_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\equiclass[2]{{#1}{[\{{#2}\}]}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\aritysugarsymbol{\rightarrow}
\mathcommand\aritysugar{\ \aritysugarsymbol\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\monus{\mathchoice
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     display-style
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     text-style
{\raisebox{-.3ex}{$\scriptstyle\dot{\raisebox{.3ex}[0ex]
{$\scriptstyle-$}}$}}                                %     scriptstyle
{\raisebox{-.2ex}{$\scriptscriptstyle\dot{\raisebox{.2ex}[0ex]
{$\scriptscriptstyle-$}}$}}                          %scriptscriptstyle
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\yields{\;\vdash\;}
\mathcommand\antiyields{\;\dashv\;}
\mathcommand\tightyields{\vdash}
\mathcommand\tightantiyields{\dashv}
\mathcommand\notyields{\;\nvdash\;}
\mathcommand\refltransyields{\hspace{0.5em}\raisebox{1.3ex}{\math{\scriptstyle
  \ast}}\hspace{-1.0em}\yields}
\mathcommand\transyields
{\hspace{0.5em}\raisebox{1.3ex}{$\scriptscriptstyle%\oplus
+$}\hspace
{-1.0em}\yields\hspace{0.3em}}
\mathcommand\notmodels{\:\not\!\models}

\newcommand\EVALSYM{{\rm eval}}
\mathapplycommand\EVAL{\EVALSYM}
\mathcommand\formerlycalledepsilon{\ident e}
\mathcommand\V{{\rm V}}
\mathcommand\X{{\rm X}}
\newcommand\nottight{\bigmath}
\mathcommand\refltransclosureinline[1]{{#1}^\ast}
\mathcommand\VARSYM {\mathcal{V}}
\mathapplycommand\VAR{\VARSYM}
\mathcommand\VARnoparentheses[1]{\VARSYM #1}
\mathcommand\VARsingleindex[1]{\VARSYM\!_{{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ZAHLENMENGEN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \N        Set of natural numbers
% \posN     Set of positive natural numbers
% \ordclass Proper class of ordinal numbers
% \ZZ       Set of integers
% \Q        Set of rationals
% \RE       Set of real numbers
% \posRE    Set of positive real numbers
% \nonnegRE Set of non-negative real numbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mathcommand\N{{\rm
% %\rm must be out here because on rare occursions does not work
% %infront of the I\hskip....
% %\ifmmode%  Sind wir im Mathemodus ?
% \mathchoice{{I\hskip -2pt   N}}% display-style
%            {{I\hskip -2pt   N}}% text-style
%            {{I\hskip -1.5pt N}}% scriptstyle
%            {{I\hskip -1pt   N}}% scriptscriptstyle
% %\else\math{\rm I\hskip-2pt N}\fi
% }}
% \newcommand\ZZ{{\rm\ifmmode\mathchoice{{Z\hskip -4pt Z}}{{Z\hskip -4pt Z}}
% {{Z\hskip -3pt Z}}{{Z\hskip -3pt Z}}\else\mbox{\tenrm Z\hskip-4pt Z}\fi}}
\mathcommand\N{{\bf N}}
\mathcommand\posN{\N_{\:\!\!\mbox{\sixsf+}}}
\mathcommand\ZZ{{\bf Z}}
\mathcommand\Q{{\bf Q}}
\mathcommand\ordclass{\mathcal{O}}
%\newcommand\RE{{\rm\ifmmode\mathchoice{{I\hskip -2pt R}}{{I\hskip -2pt R}}
%{{I\hskip -1.5pt R}}{{I\hskip -1pt R}}\else{\tenrm I\hskip-2pt R}\fi}}
\mathcommand\RE{{\bf R}}
\mathcommand\posRE{\RE_{\scriptscriptstyle +}}
\mathcommand\nonnegRE{\RE_{\scriptscriptstyle\succeq0}}

\mathcommand\Qzero{{\cal Q}_0}
\newcommand\squaredot{\,\rule{0.4ex}{0.4ex}\,}

%Transitive closures
\mathcommand\transclosure[1]{\stackrel{\scriptscriptstyle+}{#1}}
\mathcommand\transclosureinline[1]{{#1}^{\scriptscriptstyle+}}

%_____________________________________________________________________________
%Signatures
\mathcommand\sigarity{\alpha}
\newcommand\sig{{\rm sig}}
\mathcommand\sigsorts  {{\mathbb S}}
\mathcommand\sigfunsym {{\mathbb F}}
\mathcommand\consfunsym{{\mathbb C}\,} 
% \, cures strange dvips bugg
\mathcommand\deffunsym {{\mathbb N}}
\mathcommand\Ax{\mathcal{AX}}

%from header.tex
%_____________________________________________________________________________
%Reduction relation

%\red...
%\notred
%\redpara
%\revpara
%\simpara
%\unired
\mathcommand\unired{\Longrightarrow}
\mathcommand\redsimple{\longrightarrow}
\mathcommand\redindex[1]{\redsimple_{_{\!#1}}}
\mathcommand\notredindex[1]{\,\,\,\not\!\!\!\!\redsimple_{_{\!#1}}}
\newcommand\redsub             {\redindex{\R ,\X        }}
\newcommand\redsubprime        {\redindex{\R',\X'       }}
\newcommand\redshortsub        {\redindex{\R ,\V        }}
\newcommand\redshortsubprime   {\redindex{\R',\V'       }}
\newcommand\redsubY            {\redindex{\R ,\Y        }}
\newcommand\redsubemptyset     {\redindex{\R ,\emptyset }}
\newcommand\redsubprimeemptyset{\redindex{\R',\emptyset }}
\newcommand\redsubVsig         {\smallfootroom\redindex{\R ,\Vsig     }}
\newcommand\redsubVsigprime    {\smallfootroom\redindex{\R',\Vsigprime}}
\mathcommand\redindexn[2]{\stackrel{#1}\redsimple_{_{\!#2}}}
\mathcommand\redparaindex[1]{\redpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\revparaindex[1]{\revpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\simparaindex[1]{\simpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\uniredindex[1]{\unired_{\hskip-1.5pt\scriptscriptstyle#1}}

%\antired...
%\notantired..
%\antiredpara...
%\antirevpara...
%\antiunired...
\mathcommand\antiunired{\Longleftarrow}
\mathcommand\antired{\longleftarrow}
\mathcommand\antiuniredindex[1]{\antiunired_{_{\!#1}}}
\mathcommand\antiredindex[1]{\antired_{_{\!#1}}}
\mathcommand\notantiredindex[1]{\,\,\,\not\!\!\!\!\antired_{_{\!#1}}}
\newcommand\antiredsub          {\antiredindex{\R ,\X }}
\newcommand\antiredshortsub     {\antiredindex{\R ,\V }}
\newcommand\antiredshortsubprime{\antiredindex{\R',\V'}}
\newcommand\antiredsubVsig      {\smallfootroom\antiredindex{\R',\Vsig}}
\mathcommand\antiredindexn[2]{\stackrel{#1}\antired_{_{\!#2}}}
\mathcommand\antiredparaindex
[1]{\antiredpara_{\hskip-1.25pt\scriptscriptstyle#1}}
\mathcommand\antirevparaindex[1]
{\antirevpara_{\hskip-1.25pt\scriptscriptstyle#1}}

%\sym...
\mathcommand\sym{\longleftrightarrow}
\mathcommand\symindex[1]{\sym_{_{\!#1}}}
\mathcommand\symindexn[2]{\stackrel{#1}{\sym_{_{\!#2}}}}
\newcommand\symsub     {\symindex{\R,\X}}
\newcommand\symshortsub{\symindex{\R,\V}}
\newcommand\symsubVsig {\smallfootroom\symindex{\R,\Vsig}}

%Reflexive transitive closures
%Congruences
%\congru...
%\footnotecongru...
%\notcongru...
\mathcommand\refltransclosure[1]{\stackrel{\scriptstyle\ast}{#1}}
%{\mathop{#1}^{\scriptstyle\ast}}
\mathcommand\congru{\refltransclosure\sym}
\mathcommand\congruindex[1]{\congru_{_{\!#1}}}
\newcommand\congrusub             {\congruindex{\R ,\X            }}
\newcommand\congrushortsub        {\congruindex{\R ,\V            }}
\newcommand\congrusubVsig         {\smallfootroom\congruindex{\R ,\Vsig     }}
\newcommand\congrusubVsigprime    {\smallfootroom\congruindex{\R',\Vsigprime}}
\newcommand\congrusubemptyset     {\congruindex{\R ,\emptyset     }}
\newcommand\congrusubprimeemptyset{\congruindex{\R',\emptyset     }}
\mathcommand\footnotecongru%{\stackrel\footnoteoast\sym}
{\congru}
\mathcommand\footnotecongruindex[1]{\footnotecongru_{_{#1}}}
\mathcommand\notcongru{\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\sym}
\mathcommand\notcongruindex[1]{\notcongru_{_{\!#1}}}
\newcommand\notcongrusub        {\notcongruindex{\R,\X       }}
\newcommand\notcongrusubemptyset{\notcongruindex{\R,\emptyset}}

%Transitive closures
%\trans...
%\antitrans...
\mathcommand\trans{\transclosure\redsimple}
\mathcommand\transindex[1]{\trans_{_{\!#1}}}
\newcommand \transsub        {\transindex{\R,\X}}
\newcommand \transshortsub   {\transindex{\R,\V}}
\newcommand \transsubVsig    {\smallfootroom\transindex{\R,\Vsig}}
\newcommand \transsubemptyset{\transindex{\R,\emptyset}}
\mathcommand\antitrans{\transclosure\antired}
\mathcommand\antitransindex[1]{\antitrans_{_{\!#1}}}
\newcommand \antitranssub     {\antitransindex{\R,\X}}
\newcommand \antitransshortsub{\antitransindex{\R,\V}}
\newcommand \antitranssubVsig {\smallfootroom\antitransindex{\R,\Vsig}}

%Reflexive and transitive closures
%\refltrans...
%\footnoterefltrans...
%\notrefltrans...
%\antirefltrans...
%\footnoteantirefltrans...
\mathcommand\refltrans{\refltransclosure\redsimple}
\mathcommand\refltransindex[1]{\refltrans_{_{\!#1}}}
\newcommand \refltranssub          {\refltransindex{\R ,\X }}
\newcommand \refltranssubemptyset  {\refltransindex{\R ,\emptyset}}
\newcommand \refltranssubprime     {\refltransindex{\R',\X'}}
\newcommand \refltransshortsub     {\refltransindex{\R ,\V }}
\newcommand \refltransshortsubprime{\refltransindex{\R',\V'}}
\newcommand \refltranssubVsig      {\smallfootroom\refltransindex{\R ,\Vsig}}
\mathcommand\footnoterefltrans%{\stackrel\footnoteoast\redsimple}
{\refltrans}
\mathcommand\footnoterefltransindex[1]{\footnoterefltrans_{_{#1}}}
\newcommand \footnoterefltranssub     {\footnoterefltransindex{\R,\X}}
\newcommand \footnoterefltransshortsub{\footnoterefltransindex{\R,\V}}
\mathcommand\notrefltrans
            {\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\redsimple}
\mathcommand\antirefltrans{\refltransclosure\antired}
\mathcommand\antirefltransindex[1]{\antirefltrans_{_{\!#1}}}
\newcommand \antirefltranssub          {\antirefltransindex{\R ,\X }}
\newcommand \antirefltransshortsub     {\antirefltransindex{\R ,\V }} 
\newcommand \antirefltransshortsubprime{\antirefltransindex{\R',\V'}} 
\newcommand \antirefltranssubVsig      {\antirefltransindex{\R',\V'}} 
\mathcommand\footnoteantirefltrans%{\stackrel\footnoteoast\antired}
{\antirefltrans}
\mathcommand\footnoteantirefltransindex[1]{\footnoteantirefltrans_{_{#1}}}
\newcommand \footnoteantirefltranssub     {\footnoteantirefltransindex{\R,\X}}
\newcommand \footnoteantirefltransshortsub{\footnoteantirefltransindex{\R,\V}}

%joinability
\mathcommand\downarrowindex[1]{\downarrow_{_{#1}}}
\newcommand \downarrowsub        {\downarrowindex{\R ,\X       }}
\newcommand \downarrowsubemptyset{\downarrowindex{\R ,\emptyset}}
\newcommand \downarrowsubVsig    {\smallfootroom\downarrowindex{\R,\Vsig}}
\newcommand \downarrowsubprimeemptyset{\downarrowindex{\R',\emptyset}}
\mathcommand\notconfluindex[1]{\notconflu_{_{#1}}}
\newcommand \notconflusub        {\notconfluindex{\R,\X       }}
\newcommand \notconflusubemptyset{\notconfluindex{\R,\emptyset}}
\mathcommand\footnotenotconfluindex[1]{\footnotenotconflu_{_{#1}}}
\newcommand \footnotenotconflusub{\footnotenotconfluindex{\R,\X}}

%strong joinability
\mathcommand\downdownarrow        {\downdownarrows}
\mathcommand\downdownarrowindex[1]{\downdownarrow_{_{#1}}}
\newcommand \downdownarrowsub     {\downdownarrowindex{\R ,\X       }}

\mathcommand\reflclosure[1]{\stackrel
%{\raisebox{0.1em}{$\scriptscriptstyle\preceq$}{ 1}}
{\scriptscriptstyle=}
{#1}}
\mathcommand\reflclosureinline[1]{{#1}^{\scriptscriptstyle=}}
\mathcommand\onlyonce
%{{\displaystyle\mathop{\redsimple}^{{\leq}1}}}
{\reflclosure\redsimple}
\mathcommand\antionlyonce{\reflclosure\antired}
\mathcommand\onlyonceindex[1]{\onlyonce_{_{\!#1}}}
\mathcommand\antionlyonceindex[1]{\antionlyonce_{_{\!#1}}}

\mathapplycommand\nf{\rm NF}

\mathcommand\toconditiontermssub     {\twoheadrightarrow_{_{\R,\X}}}
\mathcommand\toconditiontermssubY    {\twoheadrightarrow_{_{\R,\Y}}}
\mathcommand\toconditiontermsshortsub{\twoheadrightarrow_{_{\R,\V}}}

%_____________________________________________________________________________
%Variables notation
\newcommand \U{{\rm U}}
\newcommand \Y{{\rm Y}}
\newcommand \Z{{\rm Z}}
\mathcommand\Xprime{{\rm X}'}
\mathcommand\Yprime{{\rm Y}'}
\mathcommand\Xprimeprime{{\rm X}''}
\newcommand \SIG     {{\rm SIG}}
\mathcommand\CONS    {\mathcal{C}}
\mathcommand\SIGsort     [1]{(\SIG     ,#1)}
\mathcommand\CONSsort    [1]{(\CONS    ,#1)}
\mathcommand\varsigmasort[1]{(\varsigma,#1)}
\mathcommand\SIGsortindex     [1]{_{\SIG ,#1}}
\mathcommand\CONSsortindex    [1]{_{\CONS,#1}}
\mathcommand\DUNNOsortindex   [1]{_{\DUNNO,#1}}
\mathcommand\varsigmasortindex[1]{_{\varsigma,#1}}
\mathcommand\Vsig      {\V \!_{\SIG }}
\mathcommand\Xsig      {\X   _{\SIG }}
\mathcommand\Vcons     {\V \!_{\CONS}}
\mathcommand\Sigmacons {\Sigmaoffont_{\CONS}}
\mathcommand\Xcons     {\X   _{\CONS}}
\mathcommand\Vconsprime{\V'\!_{\CONS}}
\mathcommand\Vsigprime {\V'\!_{\SIG }}
\mathcommand\sigV      {\Vsig\!\uplus\!\Vcons}
\mathcommand\sigVprime {\Vsigprime\!\uplus\!\Vconsprime}
\mathcommand\hiddenVindi     [2]{\V   \!_{{#1},{#2}}}
\mathcommand\hiddenXindi     [2]{\X     _{{#1},{#2}}}
\mathcommand\hiddenVprimeindi[2]{\V'\!\!_{{#1},{#2}}}
\newcommand \Vsigindex     [1]{\hiddenVindi\SIG     {#1}}
\newcommand \Xsigindex     [1]{\hiddenXindi\SIG     {#1}}
\newcommand \Vconsindex    [1]{\hiddenVindi\CONS    {#1}}
\newcommand \Xconsindex    [1]{\hiddenXindi\CONS    {#1}}
\newcommand \Vvarsigmaindex[1]{\hiddenVindi\varsigma{#1}}
\newcommand \Xvarsigmaindex[1]{\hiddenXindi\varsigma{#1}}
\mathapplycommand\VARCONS{\VARsingleindex\CONS}
\mathapplycommand\VARSIG {\VARsingleindex\SIG}
\mathapplycommand\VARord {\VARsingleindex\boldless}

%_____________________________________________________________________________
%Term notation
\mathcommand\vt{\mathcal{ T}}
\mathcommand\gt{\mathcal{GT}}
\mathcommand\hiddenvtindi[2]{\mathcal{ T}\!_{#1,#2}}
\mathcommand\hiddengtindi[2]{\mathcal{GT}\!_{#1,#2}}
\newcommand\vtsigindex     [1]{\hiddenvtindi{\SIG     }{#1}}
\newcommand\vtconsindex    [1]{\hiddenvtindi{\CONS    }{#1}}
\newcommand\vtvarsigmaindex[1]{\hiddenvtindi{\varsigma}{#1}}
\newcommand\gtsigindex     [1]{\hiddengtindi{\SIG     }{#1}}
\newcommand\gtconsindex    [1]{\hiddengtindi{\CONS    }{#1}}
\newcommand\gtvarsigmaindex[1]{\hiddengtindi{\varsigma}{#1}}
\mathapplycommand\hiddentv     {\mathcal{T}}
\mathapplycommand\hiddentg     {\mathcal{GT}}
\mathapplycommand\hiddentvprime{\mathcal{T}'}
%ground term sets
\newcommand\tgcons              {\hiddentg\cons }
\newcommand\tgsig               {\hiddentg\sig  }   
\newcommand\tgdunno             {\hiddentg\dunno}
\newcommand\tgconsprime         {\hiddentg{\cons'}}
\newcommand\tgsigprime          {\hiddentg{\sig' }}
\newcommand\tgunderlinecons     {\hiddentg{\underline{\underline{\cons }}}}
\newcommand\tgunderlineconsprime{\hiddentg{\underline{\underline{\cons'}}}}
%non-ground term sets
% variables from \Vsig or \Vsigprime
\newcommand\tsigV        {\hiddentv{\sig  ,\V}}
\newcommand\tsigVsig     {\hiddentv{\sig  ,\Vsig}}
\newcommand\tsigVsigprime{\hiddentv{\sig' ,\Vsigprime}}
% variables from \Vcons 
\newcommand\tcc{\hiddentv{\cons,\Vcons}}
% variables from \Vcons\cup\Vsig etc.
\newcommand\tss          {\hiddentv{\sig  ,\sigV     }}
\newcommand\tcs          {\hiddentv{\cons ,\sigV     }}
\newcommand\tcsprime     {\hiddentv{\cons',\sigVprime}}
% variables from \X or \X' etc.
\newcommand\tsigX        {\hiddentv{\sig ,\X }}
\newcommand\tconsX       {\hiddentv{\cons,\X }}
\newcommand\tsigXprime   {\hiddentv{\sig',\X'}}
\newcommand\tconsXprime  {\hiddentv{\cons',\X'}}
\newcommand\tconsVconsX  {\hiddentv{\cons,\Xcons}}
% variables from \Y
\newcommand\tsigY        {\hiddentv{\sig ,\Y }}
\newcommand\tconsY       {\hiddentv{\cons,\Y }}
%term algebras
\newcommand\tconsXalt {\app{{\mathcal T}_\CONS}\X}
\newcommand\tconsValt {\app{{\mathcal T}_\CONS}\V}
\newcommand\tX        {\hiddentv\X}
\newcommand\tXprime   {\hiddentv{\X'}}
\newcommand\tV        {\hiddentv\V}
\newcommand\tY        {\hiddentv\Y}
\newcommand\temptyset {\hiddentv\emptyset}
\newcommand\tVsig     {\hiddentv\Vsig}
\newcommand\tVsigprime{\hiddentvprime\Vsigprime}
% \newcommand{\gtc}{\hiddentg{\cons}}
%_____________________________________________________________________________
%substitutions
\mathcommand\SUBSYM{\mathcal{SU\hspace{-.08em}B}}
\mathdoubleapplycommand\SUBST{\SUBSYM}
\newcommand \Xsubst     {\SUBST\V\tX   }
\newcommand \Vsubst     {\SUBST\V\vt   }
\newcommand \Vsigsubst  {\SUBST\V\tVsig}
\newcommand \Gsubst     {\SUBST\V\gt   }
\mathcommand\Isubst     {{\rm CGSUB}(\V ,\cons )}
\mathcommand\Isubstprime{{\rm CGSUB}(\V',\cons')}
\mathcommand\GENSYM     {\mathcal{G\hspace{-.04em}E\hspace{-.09em}N}}
\mathcommand\GSSYM      {{\GENSYM\hspace{-.14em}}\SUBSYM}
\mathdoubleapplycommand\GS{\GSSYM}
\newcommand\VGS{\GS\V\vt}
\newcommand\XGS{\GS\V\tX}
\newcommand\VsigGS{\GS\V\tVsig}
%
\mathcommand\POSSYMBOL{\mathcal{P\hspace{-.08em}O\hspace{-.1em}S}}
\mathcommand\VPOSSYMBOL{\V\hspace{-.04em}\POSSYMBOL}
\mathcommand\FPOSSYMBOL{\sigfunsym\hspace{-.04em}\POSSYMBOL}
\mathapplycommand\TPOS{\POSSYMBOL}
%\mathapplycommand\POS{\POSSYMBOL} \POS is also used by xy. Use \TPOS instead!
\mathapplycommand\VPOS{\VPOSSYMBOL}
\mathapplycommand\FPOS{\FPOSSYMBOL}
%\mathcommand\OCCSYMBOL{\mathcal{O}}
%\mathapplycommand\OCC{\OCCSYMBOL}%obsolete but still in use
\mathcommand\neitherprefixsymbol{\parallel}
\mathcommand\neitherprefix[2]{{#1}\,\neitherprefixsymbol\,{#2}}
\mathcommand\replsuffix   [2]{[\,#1\leftarrow#2\,]}      %use \repl if possible
\mathcommand\replparsuffix[3]{\replsuffix{#1}{#2\ |\ #3}}%use \replpar
\mathcommand\repl         [3]{#1\penalty-1\replsuffix{#2}{#3}}
\mathcommand\replpar      [4]{#1\penalty-1\replparsuffix{#2}{#3}{#4}}
\mathcommand\eqvariablessig[1]{\mbox{\rm Eq}(\sig,{#1})}
\newcommand\eqvsig{\eqvariablessig{\sigV}}
\mathcommand\eqgsig{\mbox{\rm GEq}(\sig)}
\mathcommand\direqv[1]{\mbox{\rm DEq}(#1)}
\newcommand\direqvariablessig[1]{\direqv{\sig,{#1}}}
\newcommand\direqvsig{\direqv{\sig,\sigV}}
\mathapplycommand\MGU{\rm Mgu}
\mathdoubleapplycommand\minmgu{\rm mgu}
\mathdoubleapplycommand\sep{\rm Sep}
\mathdoubleapplycommand\minsep{\rm sep}
\mathapplycommand\depth{\rm depth}
\mathapplycommand\size{\rm size}
\newcommand\monotonic           {\tsigX-mono\-tonic}
\newcommand\Vmonotonic          {\vt-mono\-tonic}
%\newcommand\amonotonic          {an \X-mono\-tonic}
\newcommand\emptysetmonotonic   {\gt-mono\-tonic}
\newcommand\monotonicity        {\tsigX-mono\-toni\-city}
\newcommand\Vmonotonicity       {\vt-mono\-toni\-city}
%\newcommand\Monotonicity        {\X-mono\-toni\-city}
\newcommand\stable              {\X-stable}
\newcommand\Vstable             {\V-stable}
\newcommand\Ystable             {\Y-stable}
\newcommand\emptysetstable      {\mbox{$\emptyset$}-stable}
\newcommand\stability           {\X-stabi\-lity}
\newcommand\Stability           {\X-stabi\-lity}
\newcommand\Vstability          {\V-stabi\-lity}
\newcommand\VStability          {\V-stabi\-lity}
\newcommand\compatible          {\X-compa\-tible}
\newcommand\RXcompatible        {\RX-compa\-tible}
\newcommand\Vcompatible         {\V-compa\-tible}
\newcommand\Ycompatible         {\Y-compa\-tible}
\newcommand\leftrightcompatible {\X-left-right-compa\-tible}
\newcommand\Vleftrightcompatible{\V-left-right-compa\-tible}
\newcommand\dontcarecompatible  {\X-don't-care-compa\-tible}
\newcommand\aleftrightcompatible{an \X-left-right-compa\-tible}
\newcommand\adontcarecompatible {an \X-don't-care-compa\-tible}
\newcommand\compatibility       {\X-compa\-ti\-bility}
\newcommand\dontcarecompatibility{\X-don't-care-compa\-ti\-bility}
\newcommand\Vdontcarecompatible {\V-don't-care-compa\-tible}
\newcommand\Safety              {Safeness}
\newcommand\safety              {safeness}
\newcommand\safe                {safe}
\newcommand\Safe                {Safe}
\newcommand\unsafe              {unsafe}
\newcommand\safely              {safely}
\newcommand\constructorminimal{con\-struc\-tor-mini\-mal}
\newcommand\ConstructorMinimal{Con\-struc\-tor-Mini\-mal}
\newcommand\constructorminimality{con\-struc\-tor-mini\-mal\-ity}
\newcommand\constructorminimum{con\-struc\-tor-mini\-mum}
\newcommand\constructorpreserving{con\-struc\-tor-pre\-serving}
\newcommand\constructorpreservation{con\-struc\-tor-pre\-serva\-tion}
\newcommand\constructorbased{con\-struc\-tor-based}
\newcommand\Constructorbased{Con\-struc\-tor-based}
\newcommand\terminationpair{termi\-na\-tion-pair}
\newcommand\TerminationPair{Termi\-na\-tion-Pair}
\newcommand\inductivesubstitution{constructor ground substitution}
\newcommand\aninductivesubstitution{a constructor ground substitution}
\newcommand\Inductivesubstitution{Constructor ground substitution}
\newcommand\InductiveSubstitution{Constructor Ground Substitution}
\newcommand\inductiveinstance{constructor ground instance}

%Subterm
\newcommand\hiddensubST{_{_{\rm ST}}}
\mathcommand\superterm   {\rhd\hiddensubST}
\mathcommand\notsuperterm{\ntriangleright\hiddensubST}
\mathcommand\subterm     {\lhd\hiddensubST}
\mathcommand\notsubterm  {\ntriangleleft\hiddensubST}
\mathcommand\supertermeq {\trianglerighteq\hiddensubST}
\mathcommand\subtermeq   {\trianglelefteq\hiddensubST}

\mathcommand\sugarregel{l\boldequal r\rulesugar C}
\mathcommand\sugarregelindex[1]{l_{#1}\boldequal r_{#1}\rulesugar C_{#1}}
\mathcommand\sugaruncondregelindex[1]{l_{#1}\boldequal r_{#1}}
\mathcommand\ndrulewithassumption[3]{{{{\scriptstyle\lbrack}#1{\scriptstyle
\rbrack}}\atop\scriptstyle #2}\over #3}

%_____________________________________________________________________________
%Rules
\def\R{{\rm R}}
\mathcommand\RCONS{\R_\CONS}
\mathcommand\Rprime{{\rm R}'}
\mathcommand\RX{\R,\X}
\mathcommand\RCONSX{\RCONS,\X}
\mathcommand\DEFUNSYM{\mathcal{DEFUN}}
\mathapplycommand\DEFUN{\DEFUNSYM}
\newcommand\defsort{{\rm def}}
\mathcommand\ATSYM  {\mathcal{A\hspace{-.02em}T}}
\mathdoubleapplycommand\atomsof{\ATSYM}
\newcommand\atoms      {\atomsof\sig\V}
\newcommand\Xatoms     {\atomsof\sig\X}
\newcommand\Yatoms     {\atomsof\sig\Y}
\newcommand\scatoms    {\atomsof\sig\Vcons}
\mathcommand\GENATSYM  {\GENSYM\hspace{-.18em}\ATSYM}
\mathdoubleapplycommand\genatomsof{\GENATSYM}
\newcommand\genatoms      {\genatomsof\sig\V}
\newcommand\Xgenatoms     {\genatomsof\sig\X}
\newcommand\Ygenatoms     {\genatomsof\sig\Y}
\mathcommand\CONDSYM  {\mathcal{C\hspace{-.1em}O\hspace{-.12em}N\hspace{-.12em}D}}
\mathcommand\LITSYM   {\mathcal{LI\hspace{-.04em}T}}
\mathcommand\CONDLITSYM{\CONDSYM\hspace{-.04em}\LITSYM}
\mathapplycommand\condlitwitharg{\CONDLITSYM}
\newcommand\condlit {\condlitwitharg{\sig,\V}}
\newcommand\Xcondlit{\condlitwitharg{\sig,\X}}
\newcommand\Ycondlit{\condlitwitharg{\sig,\Y}}
\mathdoubleapplycommand\literals{\LITSYM}
\newcommand \lit        {\literals\sig\V}
\newcommand \Xlit       {\literals\sig\X}
\newcommand \Ylit       {\literals\sig\Y}
\mathcommand\GENLITSYM{\GENSYM\hspace{-.08em}\LITSYM}
\mathdoubleapplycommand\genliterals{\GENLITSYM}
\newcommand \genlit        {\genliterals\sig\V}
\newcommand \Xgenlit       {\genliterals\sig\X}
\newcommand \Ygenlit       {\genliterals\sig\Y}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

